Effective Resistances in Non-Expander Graphs

Effective resistances are ubiquitous in graph algorithms and network analysis. In this work, we study sublinear time algorithms to approximate the effective resistance of an adjacent pair $s$ and $t$. We consider the classical adjacency list model for local algorithms. While recent works have provided sublinear time algorithms for expander graphs, we prove several lower bounds for general graphs of $n$ vertices and $m$ edges: 1.It needs $\Omega(n)$ queries to obtain $1.01$-approximations of the effective resistance of an adjacent pair $s$ and $t$, even for graphs of degree at most 3 except $s$ and $t$. 2.For graphs of degree at most $d$ and any parameter $\ell$, it needs $\Omega(m/\ell)$ queries to obtain $c \cdot \min\{d, \ell\}$-approximations where $c>0$ is a universal constant. Moreover, we supplement the first lower bound by providing a sublinear time $(1+\epsilon)$-approximation algorithm for graphs of degree 2 except the pair $s$ and $t$. One of our technical ingredients is to bound the expansion of a graph in terms of the smallest non-trivial eigenvalue of its Laplacian matrix after removing edges. We discover a new lower bound on the eigenvalues of perturbed graphs (resp. perturbed matrices) by incorporating the effective resistance of the removed edge (resp. the leverage scores of the removed rows), which may be of independent interest.

==> chapter/Proof_algorithms_for_degree_2.tex <==
\section{Proof of Approximation Algorithm for Degree 2}\label{sec:proof_of_algo_degree_2}

In this section, we prove the correctness of Algorithm~\ref{alg:exam1}. We remark that $p_k=2^{-k}$ in this section. Let us consider its expected time. For a path of length $\ell_i$, if $j=\lfloor \log_2 \ell_i/a \rfloor$, the number of expected steps on this path is at most 
\[
p_0 \cdot 2a + p_1 \cdot 4a + \cdots + p_j \cdot 2^j a + p_{j+1} \cdot \ell_i + \cdots + p_{\log n} \cdot \ell_i = 2a \cdot j + \ell_i \cdot (p_{j+1} + \cdots + p_{\log n}) = O(a \cdot \log n).
\]
Since we can start from either $s$ or $t$, the expected time is $O(\min\{d(s),d(t)\} \cdot a \cdot \log n)$.

Next we show the approximation guarantee in \eqref{eq:additive_error}. For all paths whose lengths are at most $2 a$, the algorithm gets the exact conductance $1/\ell_i$ of them. The rest paths are divided into $\log n$ groups $G_1,\ldots,G_{\log n}$. The paths in group $G_k$ have lengths between $(2^k \cdot a,2^{k+1} \cdot a]$. Assuming path $i$ is in group $k$, we define the random variable $X_i$ for estimating $1/\ell_i$:
\begin{equation*}
    X_i = 
    \left\{
        \begin{array}{ll}
            \cfrac {1} {p_k \ell_i} - \cfrac {1} {\ell_i} \qquad & \textrm{with  probability  $p_k$}, \\
            - \cfrac {1} {\ell_i} \qquad & \textrm{with  probability  $1 - p_k$}.
        \end{array}
    \right.
\end{equation*}

So $\E X_i = 0$ and $\Var X_i = \cfrac {1 - p_k} {p_k \cdot \ell_i^2} \le \cfrac {1} {p_k \cdot \ell_i^2}$. And the result of Algorithm \ref{alg:exam1} is $\tilde \rho = \sum \cfrac {1} {\ell_i} + X_i = \rho + \sum X_i$. 

Now, we calculate the approximation of group $G_k$ by Bernstein's inequality. There are two cases of $G_k$, i.e., $\sum\limits_{G_k} \cfrac 1 {\ell_i} > b$ and $\sum\limits_{G_k} \cfrac 1 {\ell_i} \le b$ for a threshold value $b = \cfrac {\delta} {\epsilon \cdot \log n}$.

\begin{lemma}[Bernstein's inequality \cite{bernstein1912ordre}]
    Let $X_1, \cdots, X_n$ be independent zero-mean random variables. Suppose that $\left| X_{i} \right|\le M$ almost surely, for all  $i$. Then, for all positive $t$, \[ \Pr \left[ \left| \sum\limits_{i=1}^{n} X_i \right| \ge t \right] \le 2 \exp \left[ - \frac{1}{4} \cdot \min \left\{  { \cfrac {t^2} {\sum\limits_{i=1}^{n} \E X_i^2}, \frac {t} { M} }  \right\}  \right]. \]
\end{lemma}

In the previous case, ${(\sum\limits_{G_k} \cfrac 1 {\ell_i})^2} / {\sum\limits_{G_k} \cfrac 1 {\ell_i^2}} \ge \frac{ (\left | G_k \right | \cdot \min_{G_k} {\ell_i} )^2} {\left | G_k \right | \cdot (\max_{G_k} {\ell_i} )^2} \ge {\left | G_k \right |} / 4 \ge 2^{k-2} \cdot a b$. The first inequality comes from $\max\limits_{G_k} {\ell_i} < 2 \min\limits_{G_k} {\ell_i}$. And the last step is implied by $b < \sum\limits_{G_k} \cfrac 1 {\ell_i} < \left | G_k \right | / (2^k \cdot a)$ since each $\ell_i > 2^k \cdot a$ in $G_k$.

Then $\sum\limits_{G_k} \E X_i^2 \le \sum\limits_{G_k} \cfrac {1} {p_k \ell_i^2} \le \frac{4}{a b} (\sum\limits_{G_k} \cfrac 1 {\ell_i})^2$, and $|X_i| \le \frac{2^k-1}{2^k \cdot a} \le \frac{1}{a}$ for all $i \in G_k$. From the above discussion, Bernstein's inequality infers that for $t = \epsilon \sum\limits_{G_k} \cfrac 1 {\ell_i}$,
\begin{align*}
    \Pr \left[ \left | \sum\limits_{G_k} X_i \right | \ge \epsilon \sum\limits_{G_k} \cfrac 1 {\ell_i}  \right] \le 2 \exp \left[ - \frac{1}{4} \min \left\{  { \frac {ab \epsilon^2} {4},  a \epsilon \sum\limits_{G_k} \cfrac 1 {\ell_i} }  \right\}  \right]  \le 2 \exp \left[ - \frac{1}{4} \min \left\{  \frac {ab \epsilon^2} {4},  a b \epsilon  \right\}  \right].
\end{align*}
The second step is by the assumption $\sum\limits_{G_k} \cfrac 1 {\ell_i} > b$.

In the latter case, $\sum\limits_{G_k} \E X_i^2 \le \sum\limits_{G_k} \cfrac 1 {p_k \ell_i^2} \le \sum\limits_{G_k} \cfrac 1 {a \cdot \ell_i} \le \cfrac {b} {a}$ with $\ell_i \ge 2^k \cdot a$ and $\sum\limits_{G_k} \cfrac 1 {\ell_i} \le b$. So
\[ 
    \Pr \left[  \left | \sum\limits_{G_k} X_i \right | \ge \frac{\delta}  {\log n}  \right] 
    \le 2 \exp \left[ - \frac{1}{4} \min \left\{  \frac{a \delta^2} {b \log^2 n}, \frac{a \delta} {\log n}  \right\}  \right].
\]

Take a union bound for all $G_k$, and recall that $b = \frac{\delta}{\epsilon \cdot \log n}$,
\begin{align*}
    & \Pr \left[ \left | \sum\limits_{i \in [d]} X_i \right | \ge \epsilon \cdot \sum\limits_{i \in [d]} \cfrac {1} {\ell_i} + \delta  \right] \\ 
    \le & 2 \log n \cdot \exp \left[ - \frac{1}{4} \min \left\{  { ab \epsilon^2 / 4,  a b \epsilon }  \right\}  \right] + 2 \log n \cdot \exp \left[ - \frac{1}{4} \min \left\{  \frac{a \delta^2}{b \log^2 n} , \frac{a \delta}{\log n}  \right\}  \right] \\
    & \qquad \qquad (\text{plug } b = \frac{\delta}{\epsilon \cdot \log n})
    \\
    \le & 2 \log n \cdot \exp \left[ - \frac{1}{4} \min \left\{  { \frac{a \delta \epsilon}{4 \log n},  \frac{a \delta}{\log n} }  \right\}  \right] + 2 \log n \cdot \exp \left[ - \frac{1}{4} \min \left\{  \frac{a \delta \epsilon}{\log n} , \frac{a \delta}{\log n}  \right\}  \right] \\ 
    \le & 4 \log n \cdot \exp \left[ -  \frac{a \delta \epsilon}{16 \log n}  \right].
\end{align*}
% + \cfrac {100 \log n} {\epsilon \delta}
When $a = \cfrac {20 \log n \cdot \log \log n} {\epsilon \delta}$, $\tilde \rho$ is a $(1+\epsilon, \delta)$-approximation of $\rho$ with probability $0.99$.

\subsection{Proof of Claim~\ref{clm:inverse_additive_error}}\label{sec:proof_additive_error}
We finish the proof of Claim~\ref{clm:inverse_additive_error} in this section. Recall that $\tilde \rho = (1\pm \epsilon) \cdot \rho \pm \delta$ for some $\rho \ge 1$.
\begin{align*}
    1/\tilde{\rho} & =\frac{1}{(1\pm\epsilon) \rho \pm \delta}   \\
    & = \frac{1}{\rho} \cdot \frac{1}{1 \pm \epsilon \pm \delta/\rho} \\
    & = \frac{1}{\rho} \cdot (1 \pm 2\epsilon \pm 2 \delta/\rho) \\
    & = (1 \pm 2 \epsilon) \frac{1}{\rho} \pm 2 \delta.
\end{align*}
